AR-TTA: A Simple Method for Real-World Continual Test-Time Adaptation

Test-time adaptation is a promising research direction that allows the source model to adapt itself to changes in data distribution without any supervision. Yet, current methods are usually evaluated on benchmarks that are only a simplification of real-world scenarios. Hence, we propose to validate test-time adaptation methods using the recently introduced datasets for autonomous driving, namely CLAD-C and SHIFT. We observe that current test-time adaptation methods struggle to effectively handle varying degrees of domain shift, often resulting in degraded performance that falls below that of the source model. We noticed that the root of the problem lies in the inability to preserve the knowledge of the source model and adapt to dynamically changing, temporally correlated data streams. Therefore, we enhance the well-established self-training framework by incorporating a small memory buffer to increase model stability and at the same time perform dynamic adaptation based on the intensity of domain shift. The proposed method, named AR-TTA, outperforms existing approaches on both synthetic and more real-world benchmarks and shows robustness across a variety of TTA scenarios. The code is available at https://github.com/dmn-sjk/AR-TTA.

==> tables/baselines_w_exemplars.tex <==



\begin{table}[h!]
\centering
\caption{Classification accuracy and average mean class accuracy (AMCA)~(\%) results for state-of-the-art methods with simple \textbf{replay method added}. The source method is a source model without adaptation.}
\label{tab:baselines_w_replay}
\vspace{2.0mm}
\scalebox{0.7}{
\begin{tabular}{l|c|cc}
\hline

\multirow{2}{*}{Method} & CIFAR10C & \multicolumn{2}{c}{CLAD-C} \\

& Mean & Mean & AMCA \\ 

\hline

Source &
56.5 & 81.3 & 57.6 \\

\hline

TENT~\cite{TENT} &
77.3 & 70.3 & 49.2 \\

EATA~\cite{eata} &
78.6 & 71.1 & 48.4 \\

CoTTA~\cite{COTTA} &
\textbf{79.9} & 72.6 & 51.0 \\

SAR~\cite{SAR} &
75.3 & 71.1 & 48.3 \\

\hline
AR-TTA (Ours) &
78.8 & \textbf{83.7} & \textbf{63.1} \\
\hline
\end{tabular}}
\end{table}


==> tables/beta_distribution.tex <==
\begin{table}[h!]
\centering
\caption{Classification accuracy~(\%) for CIFAR10C and CLAD-C tasks for different configurations of beta distribution parameters $\psi$ and $\rho$ for sampling interpolation parameter $\lambda \sim$ Beta$(\psi, \rho)$ required for mixup data augmentation. \DS{wrap table}}
\label{tab:beta_distribution}
\scalebox{0.8}{
\begin{tabular}{cc|cc}
\hline

$\psi$ & $\rho$ & CIFAR10C & CLAD-C \\ \hline
5.0 & 5.0 & 78.6 & 83.7 \\
1.0 & 5.0 & 78.6 & 81.8 \\
5.0 & 1.0 & 78.2 & 83.0 \\
2.0 & 8.0 & 74.8 & 82.0 \\
8.0 & 2.0 & 77.5 & 83.8 \\
\hline
\multicolumn{4}{c}{Ours} \\
\hline
0.4 & 0.4 & \textbf{78.8} & \textbf{83.7} \\

\hline

\end{tabular}}
\end{table}


==> tables/cifar10.1.tex <==
\begin{table}[ht!]
\centering
\caption{Classification accuracy~(\%) for the standard CIFAR10-to-CIFAR10.1 online continual test-time adaptation task.}\label{tab:cifar10.1}
\scalebox{0.8}{
% \tabcolsep3pt
\begin{tabular}{l|c}
Method & Mean \\ \hline
Source & \textbf{88.3} \\
BN stats adapt & 81.3 \\
TENT-continual~\cite{TENT} & 82.3 \\
EATA~\cite{eata} & 82.9 \\
COTTA~\cite{COTTA} & 82.3 \\
SAR~\cite{SAR} & 81.3 \\
RMT~\cite{dobler2023CVPRmeanteacher} & 83.3 \\
RMT w/o replay~\cite{dobler2023CVPRmeanteacher} & 83.7 \\
\hline

Ours (AR-TTA) w/o replay & \textbf{88.3} $_{\pm}$ \\
Ours (AR-TTA) & \textbf{88.3}$_{\pm0}$ \\
\hline
\end{tabular}}
\end{table}


==> tables/each_component.tex <==

\begin{table}[h!]
\centering
\caption{Classification accuracy~(\%) for CIFAR10C and CLAD-C tasks for different configurations of the proposed method.}
\label{tab:each_component}
\scalebox{0.55}{
\begin{tabular}{l|c|c}
\hline
Method & CIFAR10C & CLAD-C \\
\hline
\textbf{A}: Weight-avg. teacher & 75.7$_{\pm0.07}$ & 71.1$_{\pm0.53}$ \\
\textbf{B}: A + Replay memory & 77.3$_{\pm0.16}$ & 69.0$_{\pm0.66}$ \\
\textbf{C}: B + Mixup & 78.5$_{\pm0.13}$ & 72.2$_{\pm0.31}$ \\
\hline
\textbf{D}: A + Dynamic BN stats & 77.3$_{\pm0.07}$ & 83.8$_{\pm0.82}$ \\
\textbf{E}: D + Replay memory & 79.8$_{\pm0.03}$ & 82.8$_{\pm1.09}$ \\
\hline
\textbf{AR-TTA (Ours)}: E + Mixup & 78.8$_{\pm0.13}$ & 83.7$_{\pm0.64}$ \\
\hline
\end{tabular}}
\end{table}

